Learning to Diagnose with LSTM Recurrent Neural Networks

Clinical medical data, especially in the intensive care unit (ICU), consist of multivariate time series of observations. For each patient visit (or episode), sensor data and lab test results are recorded in the patient's Electronic Health Record (EHR). While potentially containing a wealth of insights, the data is difficult to mine effectively, owing to varying length, irregular sampling and missing data. Recurrent Neural Networks (RNNs), particularly those using Long Short-Term Memory (LSTM) hidden units, are powerful and increasingly popular models for learning from sequence data. They effectively model varying length sequences and capture long range dependencies. We present the first study to empirically evaluate the ability of LSTMs to recognize patterns in multivariate time series of clinical measurements. Specifically, we consider multilabel classification of diagnoses, training a model to classify 128 diagnoses given 13 frequently but irregularly sampled clinical measurements. First, we establish the effectiveness of a simple LSTM network for modeling clinical data. Then we demonstrate a straightforward and effective training strategy in which we replicate targets at each sequence step. Trained only on raw time series, our models outperform several strong baselines, including a multilayer perceptron trained on hand-engineered features.

==> multilabel-evaluation.tex <==
F1 score, the harmonic mean between precision ($\mbox{tp}/(\mbox{tp}+\mbox{fp})$) and recall ($\mbox{tp}/(\mbox{tp}+\mbox{fp})$)
is a popular choice of performance metric when classes are imbalanced.
In terms of the entries of the confusion matrix,
$\mbox{F1}=(2 \cdot \mbox{tp})/(2 \cdot \mbox{tp} + \mbox{fp} + \mbox{fn})$.
Popular multilabel variants of F1 score for the multilabel setting include micro-averaged and macro-averaged F1.
With micro averaging, we treat the entire prediction matrix as one set of predictions. Thus we take the averages of the true positives $\bar{\mbox{tp}}$, false positives and false negatives across all labels before computing $\mbox{F1}_{\mbox{micro}}=(2 \cdot \bar{\mbox{tp}})/(2 \cdot \bar{\mbox{tp}} + \bar{\mbox{fp}} + \bar{\mbox{fn}})$.
One problem with micro-averaging however, is that when the base rates of labels follow a long-tailed distribution,
there is only minimal penalty for ignoring the rarest labels altogether by predicting every example to be negative, as they contribute only a small amount to $\bar{\mbox{fn}}$.

Alternatively, with macro-averaging the F1 is calculated separately on each label and the results are averaged. 
$$\mbox{F1}_{\mbox{macro}} = \sum_{l=1}^{|L|} \mbox{F1}_l$$.
This has the advantage or requiring that the classifier do well on a large number of labels. 
However, because the range between the F1 score achieved by a blind classifier and the best classifier is far wider for rarer labels, Macro can have the effect of prioritizing the rarest labels when base rate are heterogeneously distributed. 

Another complication of F1 score is that
unlike accuracy, for which the optimal threshold is always $.5$, 
F1 has a different optimal threshold depending upon the distribution of probabilities in the prediction set. 
Further, as shown in \cite{lipton2014optimal}, when the scores given to items are calibrated probabilities, the optimal threshold to maximize F1 is precisely $1/2$ the expected value of the F1 that it achieves.
Thus when a classifier is poor and thus the maximum expected F1 is low, the threshold is low.

A choice of threshold implies a cost sensitivity. 
If we knew the relative cost $C(\mbox{fp})$ of a false positive
and $C(\mbox{fn})$ of a false negative and 
our classifier outputted calibrated probabilistic output,
it's trivial to show that the optimal threshold would be uniquely specified 
as $\alpha /(1+\alpha)$ 
where $\alpha = C(\mbox{fp})/C(\mbox{fn})$.

Thus performing well on F1 requires care to optimally select thresholds. In the case of micro-F1, this means one universal threshold, but to maximize macro-F1, one must choose a separate threshold for each label.
Thus the choice of metric results in markedly different predictions and correspondingly 
Of course, in the medical domain, 
there can be real trade-offs between false positives and false negatives, that might not align with the thresholds chosen to maximize any chosen metric.
Nevertheless, with these caveats, 
taken together and in context, 
these metrics can be a useful way to gauge the performance of a multilabel classifier when there are varying degrees of class imbalance.
Our reported numbers for all our classifiers, including baselines, have been thresholded separately to maximize each metric.

\subsection{Area Under the Receiver Operating Characteristic Curve}
In addition to F1 measures we also report area under the ROC curve.
While we'll spare the reader a belabored description of the metric,
we note that this metric too has some complications in the multilabel setting.
As with F1 we can compute AUC either by micro-averaging or macro-averaging.
In the single label binary classification case, 
a blind classifier would be expected to achieve an AUC of .5.
However, in the multilabel case with micro-averaging and heterogeneous base rates, 
a blind classifier do considerably better by predicting the most common label first,
then the second most common label second, etc. 
Thus in our reporting we show a \emph{base rate} classifier that predicts in precisely this manner to calibrate expectations for what constitutes a good score.

\subsection{Precision and Recall at k}
While F1 and AUC are both useful for determining the relative quality of a classifier's predictions, 
it's not clear how precisely to interpret them in terms of a specific application.
Are the predictions which maximize micro-F1 useful for a diagnostic assistant?
Would we prefer the predictions which maximize some other measure?
How high an F1 is sufficient for a diagnostic assistant to be useful?
The answers to these questions are not clear.

To overcome this problem, 
we imagined a specific use case which might admit a more direct performance metric.
Specifically, we imagine the case 
where a doctor might want access to a short list of the $k$ most probable diagnoses.
After all, it may be reasonable to test for every single condition,
but it may be possible to test for $10$ or for $20$.
The measure of the quality of this list of length $k$ would simply be the precision 
within that list.
This is simply the fraction of the top 10 predictions across all patients that are actual positives.
This metric has all the interpretability of accuracy and requires no threshold setting strategy beyond the choice of $k$. 
In our reporting we list the precision at $10$ alongside micro-AUC, macro-AUC, micro-F1 and macro-F1.
Note that because there are considerably less than 10 diagnoses per patient, 
the best attainable precision at 10 is only .2281.
Further we report, recall at $k$ which is simply the fraction of all actual positives in the test set that appear in our $k$ predictions for each example.
For fixed $k$, precision and recall are monotonic functions. 
However, it's useful to evaluate recall in our application because recall indicates coverage. If we achieved a recall of $99\%$ it would mean that we could be quite confident that nearly any diagnosis would appear somewhere in the top $k$ suggestions, even if the majority of those predictions were actual negatives. 
